Precise Performance Analysis of the LASSO under Matrix Uncertainties

In this paper, we consider the problem of recovering an unknown sparse signal $\xv_0 \in \mathbb{R}^n$ from noisy linear measurements $\yv = \Hm \xv_0+ \zv \in \mathbb{R}^m$. A popular approach is to solve the $\ell_1$-norm regularized least squares problem which is known as the LASSO. In many practical situations, the measurement matrix $\Hm$ is not perfectely known and we only have a noisy version of it. We assume that the entries of the measurement matrix $\Hm$ and of the noise vector $\zv$ are iid Gaussian with zero mean and variances $1/n$ and $\sigma_{\zv}^2$. In this work, an imperfect measurement matrix is considered under which we precisely characterize the limiting behavior of the mean squared error and the probability of support recovery of the LASSO. The analysis is performed when the problem dimensions grow simultaneously to infinity at fixed rates. Numerical simulations validate the theoretical predictions derived in this paper.

==> References.tex <==
@article{tibshirani1996regression,
  title={Regression shrinkage and selection via the lasso},
  author={Tibshirani, Robert},
  journal={Journal of the Royal Statistical Society. Series B (Methodological)},
  pages={267--288},
  year={1996},
  publisher={JSTOR}
}

@article{ting2009sparse,
  title={Sparse image reconstruction for molecular imaging},
  author={Ting, Michael and Raich, Raviv and Hero III, Alfred O},
  journal={IEEE Transactions on Image Processing},
  volume={18},
  number={6},
  pages={1215--1227},
  year={2009},
  publisher={IEEE}
}

@article{gui2012improved,
  title={Improved sparse channel estimation for cooperative communication systems},
  author={Gui, Guan and Peng, Wei and Wang, Ling},
  journal={International Journal of Antennas and Propagation},
  volume={2012},
  year={2012},
  publisher={Hindawi Publishing Corporation}
}

@article{bishop2006pattern,
  title={Pattern recognition},
  author={Bishop, Christopher M},
  journal={Machine Learning},
  volume={128},
  pages={1--58},
  year={2006}
}

@inproceedings{stojnic2010recovery,
  title={Recovery thresholds for ℓ 1 optimization in binary compressed sensing},
  author={Stojnic, Mihailo},
  booktitle={Information Theory Proceedings (ISIT), 2010 IEEE International Symposium on},
  pages={1593--1597},
  year={2010},
  organization={IEEE}
}

@article{stojnic2013framework,
  title={A framework to characterize performance of lasso algorithms},
  author={Stojnic, Mihailo},
  journal={arXiv preprint arXiv:1303.7291},
 year={2013}
}

@article{donoho2009message,
  title={Message-passing algorithms for compressed sensing},
  author={Donoho, David L and Maleki, Arian and Montanari, Andrea},
  journal={Proceedings of the National Academy of Sciences},
  volume={106},
  number={45},
  pages={18914--18919},
  year={2009},
  publisher={National Acad Sciences}
}

@article{bayati2011dynamics,
  title={The dynamics of message passing on dense graphs, with applications to compressed sensing},
  author={Bayati, Mohsen and Montanari, Andrea},
  journal={IEEE Transactions on Information Theory},
  volume={57},
  number={2},
  pages={764--785},
  year={2011},
  publisher={IEEE}
}

@article{bayati2012lasso,
  title={The LASSO risk for Gaussian matrices},
  author={Bayati, Mohsen and Montanari, Andrea},
  journal={IEEE Transactions on Information Theory},
  volume={58},
  number={4},
  pages={1997--2017},
  year={2012},
  publisher={IEEE}
}


@article{newey1994large,
  title={Large sample estimation and hypothesis testing},
  author={Newey, Whitney K and McFadden, Daniel},
  journal={Handbook of econometrics},
  volume={4},
  pages={2111--2245},
  year={1994},
  publisher={Elsevier}
}

@article{rosenbaum2010sparse,
  title={Sparse recovery under matrix uncertainty},
  author={Rosenbaum, Mathieu and Tsybakov, Alexandre B and others},
  journal={The Annals of Statistics},
  volume={38},
  number={5},
  pages={2620--2651},
  year={2010},
  publisher={Institute of Mathematical Statistics}
}

@article{thrampoulidis2016precise,
  title={Precise error analysis of regularized M-estimators in high-dimensions},
  author={Thrampoulidis, Christos and Abbasi, Ehsan and Hassibi, Babak},
  journal={arXiv preprint arXiv:1601.06233},
  year={2016}
}

@inproceedings{thrampoulidis2015regularized,
  title={Regularized Linear Regression: A Precise Analysis of the Estimation Error.},
  author={Thrampoulidis, Christos and Oymak, Samet and Hassibi, Babak},
  booktitle={COLT},
  pages={1683--1709},
  year={2015}
}

@inproceedings{thrampoulidis2015lasso,
  title={Lasso with non-linear measurements is equivalent to one with linear measurements},
  author={Thrampoulidis, Christos and Abbasi, Ehsan and Hassibi, Babak},
  booktitle={Advances in Neural Information Processing Systems},
  pages={3420--3428},
  year={2015}
}

@inproceedings{thrampoulidis2015precise,
  title={Precise error analysis of the lasso},
  author={Thrampoulidis, Christos and Panahi, Ashkan and Guo, Daniel and Hassibi, Babak},
  booktitle={Acoustics, Speech and Signal Processing (ICASSP), 2015 IEEE International Conference on},
  pages={3467--3471},
  year={2015},
  organization={IEEE}
}

@inproceedings{abbasi2016general,
  title={General performance metrics for the LASSO},
  author={Abbasi, Ehsan and Thrampoulidis, Christos and Hassibi, Babak},
  booktitle={Information Theory Workshop (ITW), 2016 IEEE},
  pages={181--185},
  year={2016},
  organization={IEEE}
}

@inproceedings{zenaidi2016performance,
  title={Performance limits of energy harvesting communications under imperfect channel state information},
  author={Zenaidi, Mohamed Ridha and Rezki, Zouheir and Tembine, Hamidou and Alouini, Mohamed-Slim},
  booktitle={Communications (ICC), 2016 IEEE International Conference on},
  pages={1--6},
  year={2016},
  organization={IEEE}
}

@article{candes2006stable,
  title={Stable signal recovery from incomplete and inaccurate measurements},
  author={Candes, Emmanuel J and Romberg, Justin K and Tao, Terence},
  journal={Communications on pure and applied mathematics},
  volume={59},
  number={8},
  pages={1207--1223},
  year={2006},
  publisher={Wiley Online Library}
}
@article{candes2007dantzig,
  title={The Dantzig selector: Statistical estimation when p is much larger than n},
  author={Candes, Emmanuel and Tao, Terence},
  journal={The Annals of Statistics},
  pages={2313--2351},
  year={2007},
  publisher={JSTOR}
}
@article{bickel2009simultaneous,
  title={Simultaneous analysis of Lasso and Dantzig selector},
  author={Bickel, Peter J and Ritov, Ya'acov and Tsybakov, Alexandre B},
  journal={The Annals of Statistics},
  pages={1705--1732},
  year={2009},
  publisher={JSTOR}
}

@inproceedings{negahban2009unified,
  title={A unified framework for high-dimensional analysis of $ m $-estimators with decomposable regularizers},
  author={Negahban, Sahand and Yu, Bin and Wainwright, Martin J and Ravikumar, Pradeep K},
  booktitle={Advances in Neural Information Processing Systems},
  pages={1348--1356},
  year={2009}
}


@article{wainwright2009sharp,
  title={Sharp thresholds for high-dimensional and noisy sparsity recovery using -constrained quadratic programming (Lasso)},
  author={Wainwright, Martin J},
  journal={IEEE transactions on information theory},
  volume={55},
  number={5},
  pages={2183--2202},
  year={2009},
  publisher={IEEE}
}
